Hype or Heuristic? Quantum Reinforcement Learning for Join Order Optimisation

Identifying optimal join orders (JOs) stands out as a key challenge in database research and engineering. Owing to the large search space, established classical methods rely on approximations and heuristics. Recent efforts have successfully explored reinforcement learning (RL) for JO. Likewise, quantum versions of RL have received considerable scientific attention. Yet, it is an open question if they can achieve sustainable, overall practical advantages with improved quantum processors. In this paper, we present a novel approach that uses quantum reinforcement learning (QRL) for JO based on a hybrid variational quantum ansatz. It is able to handle general bushy join trees instead of resorting to simpler left-deep variants as compared to approaches based on quantum(-inspired) optimisation, yet requires multiple orders of magnitudes fewer qubits, which is a scarce resource even for post-NISQ systems. Despite moderate circuit depth, the ansatz exceeds current NISQ capabilities, which requires an evaluation by numerical simulations. While QRL may not significantly outperform classical approaches in solving the JO problem with respect to result quality (albeit we see parity), we find a drastic reduction in required trainable parameters. This benefits practically relevant aspects ranging from shorter training times compared to classical RL, less involved classical optimisation passes, or better use of available training data, and fits data-stream and low-latency processing scenarios. Our comprehensive evaluation and careful discussion delivers a balanced perspective on possible practical quantum advantage, provides insights for future systemic approaches, and allows for quantitatively assessing trade-offs of quantum approaches for one of the most crucial problems of database management systems.

==> tikz-figs/circuit.tex <==
\begin{yquant}
      qubit {\(\ket{0}\)} q;
      qubit {\raisebox{0.5em}{\(\vdots\)}\hspace{0.5em}} sep;
      qubit {\(\ket{0}\)} p;
 
      [this subcircuit box style={subCirc}, name=sc1]
      subcircuit {
        qubit {} q;
        qubit {} sep;
        qubit {} p;

        [style={draw=lfd1},name=enc1] box {
                    $\mathcolor{lfd1}{\hat{U}_{\text{enc}}}$} (q, sep, p) ;
        [style={draw=lfd1},name=var1] box {
                    $\mathcolor{lfd1}{\hat{U}_{\text{var}}}$} (q, sep, p) ;
        [style={draw=lfd2},name=enc2] box {
                    $\mathcolor{lfd2}{\hat{U}_{\text{enc}}}$} (q, sep, p) ;
        [style={draw=lfd2},name=var2] box {
                    $\mathcolor{lfd2}{\hat{U}_{\text{var}}}$} (q, sep, p) ;
        [style={draw=lfd4},name=enc3] box {
                    $\mathcolor{lfd4}{\hat{U}_{\text{enc}}}$} (q, sep, p) ;
        [style={draw=lfd4},name=var3] box {
                    $\mathcolor{lfd4}{\hat{U}_{\text{var}}}$} (q, sep, p) ;
      } (q, sep, p);
      
%      [ultra thin] barrier (-);
      [value=7mm] hspace q;
      [value=7mm] hspace sep;
      [value=7mm] hspace p;

      [this subcircuit box style={subCirc}, name=sc2]
      subcircuit {
        qubit {} q;
        qubit {} sep;
        qubit {} p;

        [style={draw=lfd1},name=enc1] box {} (q, sep, p) ;
        [style={draw=lfd1},name=var1] box {} (q, sep, p) ;
        [style={draw=lfd2},name=enc2] box {} (q, sep, p) ;
        [style={draw=lfd2},name=var2] box {} (q, sep, p) ;
        [style={draw=lfd4},name=enc3] box {} (q, sep, p) ;
        [style={draw=lfd4},name=var3] box {} (q, sep, p) ;
      } (q, sep, p);

      text { \textbf{\(\cdots\)} } (q, sep, p);
    
      [this subcircuit box style={subCirc}, name=sc3]
      subcircuit {
        qubit {} q;
        qubit {} sep;
        qubit {} p;

        [style={draw=lfd1},name=enc1] box {} (q, sep, p) ;
        [style={draw=lfd1},name=var1] box {} (q, sep, p) ;
        [style={draw=lfd2},name=enc2] box {} (q, sep, p) ;
        [style={draw=lfd2},name=var2] box {} (q, sep, p) ;
        [style={draw=lfd4},name=enc3] box {} (q, sep, p) ;
        [style={draw=lfd4},name=var3] box {} (q, sep, p) ;
      } (q, sep, p);

      [name=meas1] measure q;
      text { \vcont } sep;
      [name=meas4] measure p;
      discard q; discard sep; discard p;

      [value=0.25cm] hspace q;
      [value=0.25cm] hspace sep;
      [value=0.25cm] hspace p;
      
      [style={draw=black},name=pp] box { \rotatebox{90}{Post-Processing}} (q, sep, p);
      text { \vcont } sep;
\end{yquant}


==> tikz-figs/dimensions.tex <==
% Base dimensions (essentially, everything is derived from WIDTH)
\setlength{\WIDTH}{\linewidth}
\setlength{\HEIGHT}{0.5\WIDTH}

% Visual aesthetic dimensions
\newcommand{\innerSep}{4pt}
\newcommand{\lineDist}{2pt}

\tikzset{subCirc/.style={fill=bggray, draw=gray!20}}
\tikzset{dataStyle/.style={draw, semithick, dashed}}
\tikzset{varStyle/.style={draw, thin, solid, double}}
\tikzset{infoStyle/.style={draw, lfd3, very thick, -Stealth}}
\tikzset{stepArrow/.style={line width=2mm, gray!50,
                           -{Triangle Cap []. Fast Triangle[] Fast Triangle[]}}}

\def\circShift{1.5em}
\def\varCtrlDist{0.5cm}
\def\joNodeDist{1.0cm}
\def\vcont{\raisebox{0.5em}{\(\vdots\)}}

